Provable Uncertainty Decomposition via Higher-Order Calibration

We give a principled method for decomposing the predictive uncertainty of a model into aleatoric and epistemic components with explicit semantics relating them to the real-world data distribution. While many works in the literature have proposed such decompositions, they lack the type of formal guarantees we provide. Our method is based on the new notion of higher-order calibration, which generalizes ordinary calibration to the setting of higher-order predictors that predict mixtures over label distributions at every point. We show how to measure as well as achieve higher-order calibration using access to $k$-snapshots, namely examples where each point has $k$ independent conditional labels. Under higher-order calibration, the estimated aleatoric uncertainty at a point is guaranteed to match the real-world aleatoric uncertainty averaged over all points where the prediction is made. To our knowledge, this is the first formal guarantee of this type that places no assumptions whatsoever on the real-world data distribution. Importantly, higher-order calibration is also applicable to existing higher-order predictors such as Bayesian and ensemble models and provides a natural evaluation metric for such models. We demonstrate through experiments that our method produces meaningful uncertainty decompositions for image classification.

==> sections/intro.tex <==
Decomposing predictive uncertainty into aleatoric and epistemic components is of fundamental importance in machine learning and statistical prediction. Aleatoric uncertainty is the inherent or irreducible uncertainty in the prediction task at hand, arising from pure randomness in nature's data generating process, while epistemic uncertainty is the reducible uncertainty arising from a predictor's lack of perfect knowledge about nature. Accurate measurements of these quantities have many uses; they allow decision-makers to better interpret and trust their models' predictions, to recognize the inherent limits of prediction, and to understand where to focus their efforts in improving their models.

\GA{Should we define ``reducible'' above? Maybe in a footnote?}

% As a running example, consider a swing state in a two-party election where the aggregate vote distribution is 50-50. Suppose we are tasked with predicting how a typical voter in the state will vote. Our knowledge about the state may lead us to believe that every voter is in fact individually highly uncertain, and so we might predict 50-50 with high certainty. On the other hand, we may believe that the state is simply highly polarized, and consists of a balanced distribution of completely certain individuals. In this case we might wish to express that the typical voter is either 100-0 or 0-100, and we are uncertain which (if pressed, we would have to predict 50-50). In both cases, our overall predictive uncertainty is high. But in the first case we have no epistemic uncertainty and believe that our overall uncertainty arises entirely from the high aleatoric uncertainty inherent in each individual, whereas in the second case we believe that our overall uncertainty is entirely epistemic and there is no aleatoric uncertainty.

% \GA{I don't think this example is as illustrative as it could be---if we're predicting something about the ``typical'' voter like this, we don't have the nice property of many ``epistemic'' scenarios that the uncertainty would be fully resolved with just a little bit of additional training data (it's given that the aggregate vote distribution is 50-50, so seeing the votes of a few individuals doesn't give us any new information even in the epistemic case. To resolve our epistemic uncertainty, we would need to see multiple votes per individual whose certainty we're trying to predict, which is sort of an awkward thing to think about in this setting.). Wouldn't it make more sense for us to just be trying to predict the aggregate vote distribution directly, such that viewing just a few votes in the ``epistemic'' case would allow us to fully resolve the uncertainty between the 100-0 case and the 0-100 case? Obviously that's more unrealistic for an entire state and might sound a bit contrived for that reason, but we could maybe change this from voting to something else?}

As a running example, consider the task of predicting based on an X-ray scan whether a (potentially broken) bone will require a cast or not. Suppose a predictor assigns a certain patient a 50\% chance of needing a cast. We can consider two extreme scenarios in which this could arise. In the first scenario, the predictor may believe that the scan is inherently ambiguous (perhaps because it is grainy), and that real doctors presented with such a scan would all find it to be ambiguous. In the second scenario, the predictor may be unable to decide whether a certain mark on the scan indicates a crack (in which case a real doctor would definitely recommend a cast) or merely a scanning artifact (in which case a real doctor would never recommend a cast). Based on similar scans in its training data, the predictor may believe that the two possibilities are equally common and hence output 50\% on aggregate. In both of these scenarios, the total predictive uncertainty is the same. But in the first scenario the uncertainty arises entirely from the high aleatoric uncertainty inherent in the scan, whereas in the second the image would not actually be ambiguous to a real doctor and we can say that the predictor's uncertainty is entirely epistemic.

For any such explanation of a model's uncertainty to be trusted, it would ideally be accompanied by some meaningful semantics that tells us the real-world properties it satisfies. One of the most basic and well-studied such notions of semantics is \emph{calibration}, which requires that whenever our model predicts a certain distribution of outcomes, we actually observe that distribution of outcomes on average. In our X-ray example, our predictor would be calibrated if exactly half of all the scans it ever assigned a probability of 50\% did ultimately end up requiring casts. But this would be true regardless of which of the two cases above (i.e., 50-50 with high certainty \textit{vs.} an equal balance of 100-0 and 0-100) the predictor were in. Ordinary calibration is purely a property of total predictive uncertainty. Accordingly, we ask the following  question: \begin{quotation}
    \noindent
    \emph{Can we build a theory of calibration that allows us to meaningfully decompose our overall predictive uncertainty into epistemic and aleatoric components and give explicit semantics for these components?}
\end{quotation}

In this work we answer this question by proposing a theory of \emph{higher-order calibration}, a generalization of ordinary (first-order) calibration. Our X-ray example already suggests the essence of higher-order calibration: we would like our prediction to reflect the true distribution of hypothetical decisions by real doctors, not merely the average decision. 

In more detail, we take the view (not new to this work and common in the Bayesian literature, for example) that for a variety of reasons, we may be unsure what distribution over outcomes to predict, and that this is most naturally expressed using a distribution over possible predictions --- that is, a \emph{mixture} of predicted distributions. We are thus led to working with \emph{higher-order predictors}, which predict mixtures of distributions over outcomes rather than just single distributions. Thus in the first case of the X-ray example, we might predict a mixture concentrated entirely on the 50-50 distribution, while in the second we might predict an equal mixture of the 100-0 and 0-100 distributions. Higher-order predictors arise naturally in many settings, including in Bayesian and ensemble methods, but to our knowledge they have not been commonly studied as abstractions in their own right. We will discuss the connections to Bayesian methods and other related work in more detail in the related work section.

In a nutshell, a higher-order predictor is said to be higher-order calibrated if whenever it predicts a certain mixture of distributions, then we do observe that mixture of distributions over outcomes in aggregate. We now state our main definitions and results more formally.

\begin{figure}[t!]
  \centering
  \includegraphics[keepaspectratio, width=\textwidth]{figs/HOC_figure_8.pdf}
  \caption{\textbf{An illustration of higher-order calibration using the X-ray classification example.} We depict scenarios 1 and 2 on the top and bottom respectively. On the left, we have instances grouped together into one level set $[x]$ by the predictor in each of the two scenarios. By learning from snapshots drawn from the level set in either case, we are able to predict mixtures that match the true Bayes mixture $\pbayes([x])$.}
  \label{fig:hoc}
\end{figure}

\subsection{Main definitions and results}

Suppose nature generates random labeled data $(\x, \y) \in \calX \times \calY$, where $\calX$ denotes the instance space and $\calY$ denotes the (discrete) outcome or label space. Let the conditional distribution function $\pbayes : \calX \to \DY$ map each instance $x$ to the distribution of $\y \mid \x = x$ (where $\DY$ denotes the space of probability distributions over $\calY$). Thus each instance $x$ has some true aleatoric uncertainty, which is a measure of the inherent variability in $\pbayes(x)$ (such as the entropy). Epistemic uncertainty, by contrast, will emerge as a property purely of our predictor.
\begin{definition}[Higher-order predictors and higher-order calibration]\label{def:hop-hoc}
    A \emph{higher-order predictor} $\pred : \calX \to \DDY$ is a function that maps each instance to a distribution, or mixture, over $\DY$ (the space of such mixtures is denoted $\DDY$).
    
    Let $[\cdot]$ be a \emph{partition} of the input space into disjoint equivalence classes, with $[x] \subset \calX$ denoting the equivalence class of a given $x \in \calX$. The canonical level set partition induced by a predictor $\pred$ is given by $[x] = \{ x' \in \calX : \pred(x') = \pred(x)\}$. Let $\pbayes([x]) := \{ \pbayes(\x) \mid \x \sim [x] \}$ be the \emph{Bayes mixture} over $[x]$, with mixture components $\pbayes(\x)$ as $\x$ ranges over $[x]$. A higher-order predictor $\pred$ is said to be \emph{higher-order calibrated} wrt a partition $[\cdot]$ if for every $x$, $\pred(x) = \pbayes([x])$. (Approximate variants can be appropriately defined.)
\end{definition}
\UW{The notion of 'equivalence' here may mislead the reader. the notion of HoC is well defined for any partition}
We offer some remarks. In general, higher-order calibration may be defined with respect to any partition $[\cdot]$ of the inputs, with $[x]$ representing the equivalence class of points that are treated as functionally indistinguishable from $x$ (the most natural partition is based on the level sets of the predictor). Ideally, we would hope that the ground truth is in fact the same across all points in $[x]$, and that the prediction matches this ground truth. However, this is often too much to ask for (it is equivalent to learning $\pbayes$ exactly), and the predictor may implicitly be conflating multiple different points. Ordinary or first-order calibration would merely require that the prediction matches the \emph{average} ground truth distribution over $\x \sim [x]$. Higher-order calibration significantly strengthens this and guarantees that the prediction $\pred(x)$ --- now a mixture --- is an exact proxy for the true ``Bayes mixture'' of ground truth distributions $\pbayes(\x)$ as we range over $\x \sim [x]$. This is very powerful: any quantity defined in terms of the predicted mixture has a direct ``real-world'' interpretation as the corresponding quantity defined in terms of the Bayes mixture.


We now consider some natural decompositions of predictive uncertainty. Such decompositions have been studied before in the Bayesian literature, but higher-order calibration now gives them some clear semantics. Here we state arguably the most commonly studied such decomposition, which may be dubbed the ``mutual information decomposition''. While it can be stated in greater generality, for simplicity here we state it only for the Shannon entropy, which we view as a function $H : \DY \to \R$ given by $H(\distr) = -\sum_{y \in \calY} \distr_y \log \distr_y$.\footnote{To avoid confusion, note that we always view $H$ as taking in an object of type $\DY$. When $\Distr$ is itself a random variable, i.e.\ a random distribution, $H(\Distr)$ is also a random variable.}

\begin{definition}[The mutual information decomposition; see e.g.~\cite{houlsby2011bayesian,gal2016uncertainty}]\label{def:mutual-inf-decomp}
    Let $\pred : \calX \to \DDY$ be a higher-order predictor. Fix any instance $x \in \calX$, and let $\mix = \pred(x)$ be the predicted mixture at $x$. The induced marginal distribution of $\y$ when we draw $\Distr \sim \mix$ at random and then draw $\y \sim \Distr$ is given by $\meandistr = \ex[\Distr]$, the centroid of $\mix$. The \emph{mutual information decomposition} is as follows:
    \[
    \underbrace{H(\meandistr)}_{\text{Predictive uncertainty } \PU(x)} = \underbrace{\ex_{\Distr \sim \mix}[H(\Distr)]}_{\text{Aleatoric uncertainty estimate } \hat{\AU}(x)} + \underbrace{H(\meandistr) - \ex_{\Distr \sim \mix}[H(\Distr)]}_{\text{Epistemic uncertainty } \EU(x)}
    \]
\end{definition}

The predictive uncertainty here is the total entropy in a random outcome $\y$ drawn from a random mixture component $\Distr \sim \mix$. The aleatoric uncertainty estimate is sometimes referred to as the conditional entropy in $\y$ given the mixture component $\Distr$. The epistemic uncertainty $\EU(x)$ is precisely the mutual information between $\y$ and $\Distr$. It can also be equivalently written as a variance-like quantity, $\ex_{\Distr \sim \mix}[D\divx{\Distr}{\meandistr}]$ (namely the average divergence to the mean), where $D$ is the KL divergence.


\begin{theorem}[Main theorem: uncertainty decomposition semantics under higher-order calibration]    
    Suppose $\pred : \calX \to \DDY$ is higher-order calibrated. Fix any instance $x \in \calX$, let $\mix = \pred(x)$, and let $\meandistr = \ex_{\Distr \sim \mix}[\Distr]$. Let $\mixbayes = \pbayes([x])$ be the Bayes mixture over the level set $[x]$, and let $\meandistr_* = \ex_{\Distr_* \sim \mixbayes}[\Distr_*]$. Higher-order calibration guarantees that $\mix = \mixbayes$. Thus, in particular, the following properties hold. \begin{itemize}
        \item The aleatoric uncertainty estimate is accurate on average: \[ \hat{\AU}(x) = \ex_{\Distr \sim \mix}[H(\Distr)] = \ex_{\Distr_* \sim \mixbayes}[H(\Distr_*)] = \ex_{\x \sim [x]}[\AU(\x)], \] where $\AU(x) := H(\pbayes(x))$ is the true aleatoric uncertainty at $x$, given by the inherent entropy of $\pbayes(x)$.
        \item The epistemic uncertainty is exactly the average divergence of $\Distr_* \sim \mixbayes$ to the mean $\meandistr_*$ (or, equivalently, of the random distribution $\pbayes(\x)$ as $\x \sim [x]$): \[ \EU(x) = \ex_{\Distr \sim \mix}[D\divx{\Distr}{\meandistr}] = \ex_{\Distr_* \sim \mixbayes}[D\divx{\Distr_*}{\meandistr_*}]. \]
    \end{itemize}

    In fact, the same claim holds for every concave generalized entropy function $H$ (defined later). Moreover, in this generality there is an equivalence: these properties hold for all such $H$ iff $\pred$ is higher-order calibrated.
\end{theorem}

The important message here is the following: higher-order calibration locates the source of our epistemic uncertainty in bucketing multiple potentially different points together into a single level set $[x]$. Our quantification of epistemic uncertainty is precisely the ``variance'' in $\pbayes(\x)$ as $\x \sim [x]$. And our estimate of aleatoric uncertainty captures the average inherent entropy (or true aleatoric uncertainty) in $\pbayes(\x)$ as $\x \sim [x]$.

TODO: also state prediction intervals 

\subsection{Achieving higher-order calibration: learning from snapshots}

Higher-order calibration is clearly a strong property; how might one actually achieve it? Let us return to our X-ray example. Suppose we train a new predictor on a training set that's either composed 1. exclusively of ambiguous scans (scans that cause disagreements between doctors) or 2. of an equal mixture of completely unambiguous scans, half of which will unanimously require a cast and half of which will unanimously not.  For the sake of argument, suppose too that the predictor completely lacks the ability to distinguish scans from one another based on their features alone; perhaps buggy  data augmentation code in the predictor's pipeline obscures the most important parts of the scan. Our first crucial observation is that we cannot hope to distinguish scenario 1 from scenario 2 if all we receive are ordinary labeled examples $(\x, \y)$ where $\x$ is sampled at random from the state and $\y$ is their vote. Intuitively, since we cannot tell apart the various $\x$, we will effectively receive a 50-50 distribution of votes in both scenarios. There is no information on the basis of which to learn a higher-order calibrated predictor. The only reasonable course is to predict 50-50 for all individuals. This is the predictor that will minimize any convex loss {\bf even in scenario 2}. 

To get beyond this indistinguishability barrier, suppose that we have access to \emph{$k$-snapshots}  where  we first sample $\x$ according to nature, but we then receive $k$ independent conditional samples $\y_1, \dots, \y_k \sim \pbayes(\x)$ for each $\x$. For example, we could imagine that multiple doctors have labeled each scan. In scenario 1, we would see snapshots that tend to be quite balanced, while in scenario 2 we would only see snapshots that are either all $0$s or all $1$s. \eat{This is clearly enough information to tell the two apart.} 

As it turns out, $k$-snapshots are exactly what we need to achieve higher-order calibration. Indeed, a $k$-snapshot can be seen as a coarse representation of a distribution of outcomes (by viewing it as a histogram). A distribution over $k$-snapshots is thus a coarse representation of a mixture. By framing our goal as that of learning a $k$-snapshot predictor from $k$-snapshot examples, we obtain an effective way of learning an (approximate) higher-order predictor. In fact, the $k$-snapshot framework provides a natural way of defining a hierarchy of calibration notions, termed $k\th$-order calibration, that ranges from ordinary first-order calibration when $k=1$ to perfect higher-order calibration as $k \to \infty$. Moreover, $k\th$-order calibration is simple to define, and in essence reduces to ordinary first-order calibration over the extended label space of $k$-snapshots. This leads to a very simple and general recipe: we can leverage any general-purpose procedure guaranteeing first-order calibration over this extended label space to achieve $k\th$-order calibration. We also prove a formal statement showing that $k\th$-order calibration converges to higher-order calibration by showing that the gap in the two kinds of calibration error decays at a $1/\sqrt{k}$ rate.

TODO: figure out whether and how to state this semi-formally in the intro


It is natural to ask how strong the assumption of access to $k$-snapshots for learning is. We believe that there are several learning scenarios where one could reasonably model having such access. In a medical or crowd-sourcing setting, we can imagine showing each $\x$ to multiple experts, each of whom answers with their own label $\y_i$. We can model these $\y_i$s as independent draws from the Bayes optimal distribution. Here $k$ is decided by the number of experts we can call on. When trying to distill a larger model into a small one, we can ask for $k$-snapshots for large $k$. But not every scenario admits such access; in settings such as medical trials, any $k > 1$ might not be feasible. 

We note that the $k=2$ case of $k\th$-order calibration had already been defined and studied as second-order calibration in the recent beautiful work of \cite{johnson2024experts}. Our work builds on and considerably generalizes theirs; we discuss the connections in more detail in the related work section.

%greatly extends the notion of second-order calibration by defining the limiting notion of higher-order calibration that is implicit in their viewpoint. This allows us to view $k\th$-order calibration more generally as providing a natural hierarchy between first-order and higher-order calibration. Further connections are discussed in the related work section.

%We also leverage various techniques from recent theoretical computer science literature on calibration to build a full-fledged theory of higher-order calibration. TODO: cite

We have just described a way of learning a higher-order calibrated predictor directly from $k$-snapshots. But a key advantage of our framework is that it also allows a natural way of achieving higher-order calibration \emph{as a pure post-processing routine}, analogous to first-order calibration procedures such as Platt scaling. For this we only require a \emph{calibration set} of $k$-snapshot examples (as opposed to a full training set). Indeed, suppose we start from an ordinary first-order calibrated model (trained using ordinary 1-snapshot examples, possibly even a large pretrained model). We can consider its level set partition $[\cdot]$ (or more generally any desired partition $[\cdot]$ of the space into equivalence classes of functionally indistinguishable instances). Now, higher-order calibration wrt $[\cdot]$ entails exactly the following: for any given equivalence class $[x]$, we need to learn the true Bayes mixture $\pbayes([x])$ (with mixture components $\pbayes(\x)$ as $\x \sim [x]$). Thus we have reduced our problem to a collection of pure \emph{mixture learning} problems. This problem has been studied before in the theoretical computer science literature, and near-optimal learning algorithms are known \cite{li2015learning}. We leverage these results to provide a simple higher-order calibration procedure with near-optimal sample complexity bounds. TODO: state semi-formally or not?

%In fact, in the general case a very natural procedure turns out to be near-optimal: draw a collection of $k$-snapshots, view each $k$-snapshot as a distribution, and consider the uniform empirical mixture over these distributions.

\subsection{Related work}
\input{sections/related_work_intro}

==> sections/poly_approx.tex <==
In this section we show an alternative means of estimating the true aleatoric uncertainty under $k\th$-order calibration using polynomial approximation.

We first formally state the definition of uniformly continuous functions.

\begin{definition}[Uniform continuity and modulus of continuity]
\label{def:uniform-cont-2}
    Consider a function $G : \DY \to \R$, where we view $\DY$ as a subset of $\R^{\ell}$ equipped with the $\ell_1$ distance metric. We say that $G$ is \emph{uniformly continuous} if there exists a function $\omega_G : \R_{\geq 0} \to \R_{\geq 0}$ vanishing at $0$ such that for all $p, p' \in \DY$, we have \[ |G(p) - G(p')| \leq \omega_G(\|p - p'\|_1). \] The function $\omega_G$ is called the \emph{modulus of continuity} of $G$.
\end{definition}

\begin{remark}
\label{rem:uniform-cont}
    Uniform continuity can be usefully thought of as a relaxation of Lipschitzness. The latter is the special case where $\omega_G(\delta) \leq O( \delta)$. We will always be concerned with the behavior of $\omega_G$ for small values of $\delta \ll 1$, and in this regime we may assume without loss of generality that $\omega_G(\delta) \leq O(\delta^{\alpha})$ for some $\alpha$. Moreover, we may assume that $\alpha \leq 1$, simply because if $\alpha > 1$ then $\delta^{\alpha} \leq \delta$ (for small $\delta$). In particular, $\omega_G$ can be assumed WLOG to be a concave, non-decreasing function for small $\delta$.
\end{remark}

In the rest of this case we specialize to binary labels $\calY = \{0, 1\}$, where $\DY$ may be identified with $[0, 1]$, and $G : [0, 1] \to \R$ becomes a simple real-valued function on the unit interval. We now state Jackson's well-known theorem from approximation theory on approximating such functions using polynomials.

\begin{definition}
 We say that $G : [0, 1] \to \R$ admits a $(d, \alpha, B)$-polynomial approximation if there exists a degree $d$ polynomial
$p(t) = \sum_{i=0}^d \beta_i t^i$ such that $|\beta_i|\leq B$ for all $i$ and
\[ \sup_{t \in [0,1]} \left|p(t) - G(t)\right| \leq \alpha.\]
\end{definition}

\begin{theorem}[{Jackson's theorem; see e.g.\ \cite[Thm 1.4]{rivlin1981introduction}}]\label{thm:jacksons}
    Let $G : [0, 1] \to \R$ be a uniformly continuous function with modulus of continuity $\omega_G$. Then for any $d > 0$, $G$ admits a $(d, O(\omega_G(\frac{1}{d})), \exp(\Theta(d)))$-polynomial approximation.
\end{theorem}

The bound on the coefficients can be shown using standard bounds on the coefficients of the Chebyshev polynomials, but also holds more generally for any polynomial $F$ that is bounded on the interval (see e.g.\ \cite[Cor 2, p56]{natanson1964constructive}).

%\subsection{Applications}\label{sec:AU-poly-approx}

\AG{WIP}\todo{is this still a wip?}


We now give an alternative to \cref{thm:koc-aleatoric-approx} that can provide better error guarantees for particular choices of $G$ in regimes where $k$ is quite small, and thus the $\frac{|\calY|}{2\sqrt{k}}$ term arising in that theorem could dominate the overall error. Recall that we are working with the binary case ($\calY = \{0 ,1\}$) for simplicity.
In this case our mixture gives us a random variable on $[0, 1]$, and we have the following theorem:

\begin{theorem}\label{thm:koc-degk-aleatoric-approx}
    Let $\calY = \{0, 1\}$ and let $G : [0, 1] \to \R$ be a concave generalized entropy function that has $(d, \alpha, B)$-polynomial approximations. Then, if $\spred: \calX \rightarrow \Delta \Ysnap$ is an $\epsilon$-$k\th$-order calibrated predictor for any $k \geq d$, then for each $x \in \calX$, we can use $\spred$ to estimate $\ex_{\x \sim [x]}[\AU_G^*(\x)]$ to within an additive error $\delta = \alpha + d^2\epsilon B/2.$
\end{theorem}


To apply this theorem, we need to show that commonly used entropy functions have good polynomial approximations. We show that this is indeed the case for the examples considered earlier.  The Brier entropy or Gini impurity $G_\brier(p) = 4p(1-p)$ is trivial since it is itself a quadratic. Hence we get the following corollary:

\begin{corollary}[Corollary to Theorems~\ref{thm:koc-degk-aleatoric-approx} and~\ref{thm:sample-cxty}, Estimating Brier Entropy]
    %Let $\Y = \{0, 1\}$. Given any partition $[\cdot]$ and $x \in \calX$ and error parameters $\epsilon > 0$ and $\delta \in [0, 1]$, we can obtain an estimate $\hat{\AU_{G_{\text{Brier}}}}$ of the average aleatoric uncertainty wrt the Brier entropy $G_{\text{Brier}}(p) = 4p(1-p)$ over the partition $[x]$ using $N \geq 128(4\log(2) + \log(1/\delta))/\epsilon^2$ $2$-snapshot samples from $[x]$ such that with probability at least $1 - \delta$, 
    %\[\left|\hat{\AU_{G_{\text{Brier}}}} - \ex_{\x \sim [x]}[\AU^*_{G_{\text{Brier}}}(\pbayes(\x))]\right| \leq \epsilon.\]


    Let $\epsilon > 0$. Let $g : \calX \to \Delta \Y^{(2)}$ be an $(\epsilon/8)$-second-order calibrated predictor. Let $G_\brier(p) = 4p(1-p)$ denote the Brier entropy. Then we can use $g$ to obtain an estimate $\hat{\AU}_\brier$ such that with high probability \[\left|\hat{\AU}_\brier - \ex_{\x \sim [x]}[\AU^*_{G_{\brier}}(\pbayes(\x))]\right| \leq \epsilon.\]
    In particular, we require only $N \geq 128(4\log(2) + \log(1/\delta))/\epsilon^2$ $2$-snapshot examples from $[x]$ for this guarantee to hold with probability at least $1-\delta$.
    
\end{corollary}

\begin{proof}
    The Brier entropy presents a particularly easy case of Theorem~\ref{thm:koc-degk-aleatoric-approx} because $G_{\text{Brier}}(p) = 4p(1-p)$ is itself a polynomial of degree 2 with coefficients bounded in absolute value by 4. 

    Theorem~\ref{thm:koc-degk-aleatoric-approx} thus guarantees that an $(\epsilon/8)$-second-order calibrated predictor can estimate $\ex_{\x \sim [x]}[\AU^*_{G_{\text{Brier}}}(\pbayes(\x))]$ to within an additive error of $\epsilon$.

    Theorem~\ref{thm:sample-cxty} tells us that $N \geq 128(4\log(2) + \log(1/\delta))/\epsilon^2$ samples from $[x]$ are sufficient to guarantee an $\epsilon/8$-second-order-calibrated prediction for $[x]$ with probability at least $1-\delta$, thus giving an additive error of $\epsilon$ when estimating the aleatoric uncertainty. 
\end{proof}

\begin{corollary}[Corollary to Theorems~\ref{thm:koc-degk-aleatoric-approx} and~\ref{lem:ko-moment-approx}, Estimating Shannon Entropy]
    %Let $\Y = \{0, 1\}$. Given any partition $[\cdot]$ and $x \in \calX$ and error parameters $\epsilon > 0$ and $\delta \in [0, 1]$, we can obtain an estimate $\hat{\AU_{G_{\text{Shannon}}}}$ of the average aleatoric uncertainty wrt the Shannon entropy, $G_{\text{Shannon}}(p) = -p\log p - (1 - p)\log(1-p)$ over the partition $[x]$ using $N \geq O(\log(1/\delta)\exp(O((1/\epsilon)^{\ln 4})))$ $k = O((1/\epsilon)^{\ln 4})$-snapshot samples from $[x]$ such that with probability at least $1 - \delta$, 
    %\[\left|\hat{\AU_{G_{\text{Shannon}}}} - \ex_{\x \sim [x]}[\AU^*_{G_{\text{Shannon}}}(\pbayes(\x))]\right| \leq \epsilon.\]

    Let $\epsilon > 0$. Let $g : \calX \to \Delta \Ysnap$ be an $\epsilon'$-$k\th$-order calibrated predictor where $k \geq \Theta(\left(\frac{1}{\epsilon}\right)^{\ln 4}$), and $\epsilon' \leq \frac{\epsilon}{\exp(\Theta(k))}$. Let $G_{\shn}(p) = -p\log p - (1 - p)\log(1-p)$ denote the Shannon entropy. Then we can use $g$ to obtain an estimate $\hat{\AU}_\shn$ such that with high probability, \[\left|\hat{\AU_{\shn}} - \ex_{\x \sim [x]}[\AU^*_{G_{\shn}}(\pbayes(\x))]\right| \leq \epsilon.\]
    In particular, we require only $N \geq O(\log(1/\delta)\exp(O((1/\epsilon)^{\ln 4})))$ $k$-snapshot examples from $[x]$ for this guarantee to hold with probability at least $1-\delta$.
\end{corollary}

\begin{proof}
    The Shannon entropy $G_\shn(p) = -p \log p - (1-p)\log (1-p)$ can be dealt with using Jackson's theorem (Theorem~\ref{thm:jacksons}), which tells us that for any $d \geq 1$, there exists a degree-$d$ polynomial $F$ and constant $C_1$ such that 
    \[\sup_{x \in [0, 1]}|F(x) - G_\shn(x)| \leq C_1\omega_{G}(1/d),\]
    and the coefficients of $F$ are bounded by $\exp(C_2 d)$ for some constant $C_2$. Here $\omega_{G}$ is the modulus of continuity of $G_{\shn}$ (Definition~\ref{def:uniform-cont-2}), defined by 
    \[ \omega_G(x) = \sup \{ |G_\shn(p) - G_\shn(p')| \mid p, p' \in [0, 1],\ |p - p'| \leq x\}. \]

    In the case of the binary entropy function, it is easy to see that the supremum is achieved at the endpoints, e.g.\ at $p = 0, p' = x$, and so $\omega_G(x) = G_\shn(x)$.
    Now, it turns out that the binary entropy function satisfies the following useful bound \citep{topsoe2001bounds}: \[ G_\shn(x) \leq (4x(1-x))^{1/\ln 4} \leq (4x)^{1/\ln 4}. \] 

    Thus, to ensure $C_1\omega_{G}(1/d) \leq \epsilon/2,$ it suffices to take $k \geq d \geq \frac{1}{4}\left(\frac{2C_1}{\epsilon}\right)^{\ln 4}.$ We choose the minimal snapshot size that can achieve this, and take $k = \frac{1}{4}\left(\frac{2C_1}{\epsilon}\right)^{\ln 4}$.

    By Theorem~\ref{thm:koc-degk-aleatoric-approx}, for this value of $k$ we are guaranteed that an $\epsilon'$-$k\th$-order calibrated predictor will give estimates of the aleatoric uncertainty with additive error at most $\epsilon/2 + k^2\epsilon'e^{C_2 k}/2$. 

    Thus, there exists a constant $C_3$ such that it suffices to have $\epsilon' \leq \frac{\epsilon}{e^{C_3 k}}$ to guarantee an error of at most $\epsilon$. Plugging this bound into Theorem~\ref{thm:sample-cxty} tells us that there exists a constant $C_4$ such that $N \geq \exp(C_4 (1/\epsilon)^{\ln 4})\log(1/\delta)$ samples from $[x]$ are enough to guarantee that the $k\th$-order calibration error in that partition is at most  $\frac{\epsilon}{e^{C_3 k}}$ with probability at least $1 - \delta$, thus guaranteeing that the overall additive approximation error of estimating the Shannon entropy on $[x]$ will be at most $\epsilon$ with probability at least $1 - \delta$. 

    We complete the proof by noting that $\exp(C_4 (1/\epsilon)^{\ln 4})\log(1/\delta) = O(\log(1/\delta)\exp(O((1/\epsilon)^{\ln 4}))).$
\end{proof}





